Feature Generation for Long-tail Classification

The visual world naturally exhibits an imbalance in the number of object or scene instances resulting in a \emph{long-tailed distribution}. This imbalance poses significant challenges for classification models based on deep learning. Oversampling instances of the tail classes attempts to solve this imbalance. However, the limited visual diversity results in a network with poor representation ability. A simple counter to this is decoupling the representation and classifier networks and using oversampling only to train the classifier. In this paper, instead of repeatedly re-sampling the same image (and thereby features), we explore a direction that attempts to generate meaningful features by estimating the tail category's distribution. Inspired by ideas from recent work on few-shot learning, we create calibrated distributions to sample additional features that are subsequently used to train the classifier. Through several experiments on the CIFAR-100-LT (long-tail) dataset with varying imbalance factors and on mini-ImageNet-LT (long-tail), we show the efficacy of our approach and establish a new state-of-the-art. We also present a qualitative analysis of generated features using t-SNE visualizations and analyze the nearest neighbors used to calibrate the tail class distributions. Our code is available at https://github.com/rahulvigneswaran/TailCalibX.

==> tables/all_tables.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
Dataset                                                            & \multicolumn{3}{l}{Cifar100} \\ \midrule
Imbalance ratio                                                    & 100      & 50      & 10      \\
CE                                                                 &          &         &         \\
CosineCE                                                           &          &         &         \\
Decoupled Learning                                                 &          &         &         \\
CBD                                                                &          &         &         \\
FreeLunch(repeat(Generate once, Train Classifier once)) (Ours)     &          &         &         \\
CBD+FreeLunch(repeat(Generate once, Train Classifier once)) (Ours) &          &         &         \\ \bottomrule
\end{tabular}%
}
\caption{Final-cifar100}
\label{tab:my-table}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Dataset                                                            & \multicolumn{4}{l}{Imagenet\_LT}                          \\ \midrule
Method                                                             & Many-shot & Mid-shot & Few-shot & \multicolumn{1}{c}{All} \\
CE                                                                 &           &          &          &                         \\
Decoupled Learning                                                 &           &          &          &                         \\
CBD                                                                &           &          &          &                         \\
FreeLunch(repeat(Generate once, Train Classifier once)) (Ours)     &           &          &          &                         \\
CBD+FreeLunch(repeat(Generate once, Train Classifier once)) (Ours) &           &          &          &                        
\end{tabular}%
}
\caption{Imagenet Final}
\label{tab:my-table}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Dataset               & \multicolumn{3}{l}{Cifar100} & Imagnet\_LT           \\ \midrule
Imbalance ratio       & 100      & 50      & 10      & \multicolumn{1}{c}{-} \\
CosineCE Nothing      &          &         &         &                       \\
CosineCE relu         &          &         &         &                       \\
CosineCE Soft+ (Ours) &          &         &         &                       \\ \bottomrule
\end{tabular}%
}
\caption{CosineCE}
\label{tab:my-table}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Dataset                                    & \multicolumn{3}{l}{Cifar100} & Imagnet\_LT           \\ \midrule
Imbalance ratio                            & 100      & 50      & 10      & \multicolumn{1}{c}{-} \\
FreeLunch (with l2 norm)(with pretrain)    &          &         &         &                       \\
FreeLunch (without l2 norm)(with pretrain) &          &         &         &                      
\end{tabular}%
}
\caption{FreeLunch: (Consider only the CosineCE version)(Better features = Better generated features)}
\label{tab:my-table}
\end{table*}



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllll@{}}
\toprule
Dataset                                                         & \multicolumn{3}{l}{Cifar100} & Imagnet\_LT           \\ \midrule
Imbalance ratio                                                 & 100      & 50      & 10      & \multicolumn{1}{c}{-} \\
FreeLunch(Generate once, Train Classifier for 100 epochs)       &          &         &         &                       \\
FreeLunch(repeat(Generate once, Train Classifier once)) (Final) &          &         &         &                      
\end{tabular}%
}
\caption{FreeLunch (Training configs)}
\label{tab:my-table}
\end{table*}

